Low-Latency Graph Streaming Using Compressed Purely-Functional Trees

Due to the dynamic nature of real-world graphs, there has been a growing interest in the graph-streaming setting where a continuous stream of graph updates is mixed with arbitrary graph queries. In principle, purely-functional trees are an ideal choice for this setting due as they enable safe parallelism, lightweight snapshots, and strict serializability for queries. However, directly using them for graph processing would lead to significant space overhead and poor cache locality. This paper presents C-trees, a compressed purely-functional search tree data structure that significantly improves on the space usage and locality of purely-functional trees. The key idea is to use a chunking technique over trees in order to store multiple entries per tree-node. We design theoretically-efficient and practical algorithms for performing batch updates to C-trees, and also show that we can store massive dynamic real-world graphs using only a few bytes per edge, thereby achieving space usage close to that of the best static graph processing frameworks. To study the efficiency and applicability of our data structure, we designed Aspen, a graph-streaming framework that extends the interface of Ligra with operations for updating graphs. We show that Aspen is faster than two state-of-the-art graph-streaming systems, Stinger and LLAMA, while requiring less memory, and is competitive in performance with the state-of-the-art static graph frameworks, Galois, GAP, and Ligra+. With Aspen, we are able to efficiently process the largest publicly-available graph with over two hundred billion edges in the graph-streaming setting using a single commodity multicore server with 1TB of memory.

==> inputs/abstract.tex <==
\begin{abstract}

  Due to the dynamic nature of real-world graphs there has been
  growing interest in the streaming graph setting where a
  continuous stream of graph updates is mixed with arbitrary graph
  queries.  Existing frameworks that support this setting, however,
  either disallow queries during updates, are not serializable, have a
  large space overhead, and/or have significant update latency.

  This paper presents Aspen, a graph-streaming framework that supports
  strictly serializable low-latency queries and updates on graphs
  while only requiring a few bytes of storage per edge.  The main idea behind
  Aspen is the use of a purely functional compressed tree
  representation, which we refer to as a \treeplus.  The fact that it
  is functional allows for lightweight snapshots, so that queries
  (potentially long lasting) can proceed atomically while updates are
  happening.  The compression scheme uses a blocking technique over the
  trees and difference encoding over blocks of edges to achieve
  compression close to that of the best static graph processing frameworks.

  Aspen extends the full interface of Ligra with operations for
  updating graphs.  We show that on queries it achieves reasonable
  performance relative to Ligra, while concurrently supporting updates
  with latencies under a millisecond and throughputs in the millions
  of updates per second.  With Aspen we are able to process the
  WebDataCommons hyperlink graph with hundreds of billions of edges on
  a reasonably modest multicore with a terabyte of memory.
\end{abstract}


==> inputs/framework.tex <==
\section{Aspen}\label{sec:aspen}

In this section, we describe an interface for processing streaming
graphs. The interface is an extension of the Ligra interface with a
set of new primitives that enable a single writer to update the graph,
and concurrent readers to acquire an immutable snapshot of the graph.
Lastly, we describe an implementation of the interface using the
\treepluses{} developed in Section~\ref{sec:trees}.

%% guarantees for each
%% primitive in the interface follow directly from the algorithm
%% description in Section~\ref{
%% Finally, we describe how we use a recently developed solution to the
%% version maintenance problem to concurrently support a single (batch)
%% writer and multiple concurrent readers using possibly manay different
%% versions of the graph data structure.

\subsection{An Interface for Streaming Graphs}

%% TODO: are we defining a framework or an interface? we use the words
%% interchangably
We start by defining a few types used by the interface. A
$\mathbfsf{versioned\_graph}$ is a datatype that represents multiple
snapshots of an evolving graph. A $\mathbfsf{version}$ is a
purely-functional snapshot of a $\versionedgraph{}$. A $\mathbfsf{T} \
\mathbfsf{seq}$ is a sequence of values of type $\mathbfsf{T}$.
Finally, a $\mathbfsf{vertex}$ is a purely-functional vertex contained
in some $\version{}$.

\myparagraph{Building and Update Primitives}
The main functions in our interface are a method to construct the
initial graph, methods to acquire and release $\versions{}$, and
methods to modify a graph.  The remaining functions in the interface
are for traversing and analyzing $\versions{}$ and are similar to the
Ligra interface.  Aspen's functions are listed below:
\smallskip

%\begin{itemize}
\noindent {\textbf{\buildgraph{}}($n$ : $\mathsf{int}$, $m$ : $\mathsf{int}$,} \\
  	 \hspace*{2.20cm}$S$ : $\mathsf{int}$\ $\mathsf{seq}$\ $\mathsf{seq}$) :
     $\versionedgraph{}$\\ 
  Creates a versioned graph containing $n$ vertices and $m$
  edges. The edges incident to the $i$'th vertex are given by $S[i]$.

  \smallskip

 \noindent\textbf{\acquire{}}() : ($VG$ : $\versionedgraph{}$) : $\version{}$\\ 
  Returns a valid $\version{}$ of a $\versionedgraph{}$ $VG$.
  Note that this version will be persisted until the user calls
  \release{}.

  \smallskip

 \noindent\textbf{\release{}}() : ($VG$ : $\versionedgraph{}$, $G$ : $\version{}$) \\ 
 Releases a $\version{}$ of a $\versionedgraph{}$ $VG$.

 \smallskip

 \noindent\textbf{\insertedges{}}() : ($VG$ : $\versionedgraph{}$,
$E'$: $\mathsf{int} \times \mathsf{int}\ \mathsf{seq}$) \\ 
  Updates the latest version of the graph, $G=(V,E)$, by inserting the
  edges in $E'$ into $G$. Makes a new version of the graph equal to
  $G[E \cup E']$ visible to readers.

  \smallskip

 \noindent\textbf{\deleteedges{}}() : ($VG$ : $\versionedgraph{}$,
$E'$: $\mathsf{int} \times \mathsf{int}\ \mathsf{seq}$) \\ 
  Updates the latest version of the graph, $G=(V,E)$, by deleting the
  edges in $E'$ from $G$. Singleton vertices (those with degree $0$ in
  the new version of the graph) can be optionally removed.  Makes a
  new version of the graph equal to $G[E \setminus E']$ visible to
  readers.
  % \julian{does it delete the singleton vertices?}
  % Currently no, but it should be easy to implement this as an option
  % with a flag

  \smallskip

 \noindent\textbf{\insertvertices{}}() : ($VG$ : $\versionedgraph{}$,
$V'$: $\mathsf{int}\ \mathsf{seq}$) \\ 
  Updates the latest version of the graph, $G=(V,E)$, by inserting the
  vertices in $V'$ into $G$. Makes a new version of the graph equal to
  $G[V \cup V']$ visible to readers.

  \smallskip

 \noindent\textbf{\deletevertices{}}() : ($VG$ : $\versionedgraph{}$,
$V'$: $\mathsf{int}\ \mathsf{seq}$) \\ 
  Updates the latest version of the graph, $G=(V,E)$, by deleting the
  vertices in $V'$ from $G$. Makes a new version of the graph equal to
  $G[V \setminus V']$ visible to readers.
% I think edges was a typo here. It should be vertices.
%  \julian{does it delete the edges on $V'$ as well?}

 \smallskip

Our framework also supports similarly-defined primitives
for updating values associated with edges (e.g., edge weights) and
updating values associated with vertices (e.g., vertex weights).
%% Due
%% to space constraints we do not list them here, but
The interface is similar to
the basic primitives for updating edges and vertices.

\myparagraph{Access Primitives}
The functions for accessing a graph are defined similarly to Ligra.
For completeness, we list them below. We also provide
primitives over the $\vertex{}$ object, such as \vtxdegree{},
\vtxmap{}, and \vtxintersection{}, that we do not describe here due to
space constraints.

\smallskip

 \noindent\textbf{\numvertices{} (\numedges{})}() : ($G$ : $\version{}$)
 : $\mathsf{int}$\\ 
 Returns the number of vertices (edges) in the graph.

 \smallskip

 \noindent\textbf{\findvertex{}}() : ($G$ : $\version{}$, $v$:
 $\mathsf{int}$) : $\{\vertex{} \cup \Box \}$\\ 
 Returns either the vertex corresponding to the vertex identifier $v$,
 or $\Box$ if $v$ is not present in $G$.

 \smallskip

 \noindent\textbf{\emap{}}() : ($G$ : $\version{}$, $U$ : \vset{}, $F$: $\mathsf{int} \times \mathsf{int} \rightarrow \mathsf{bool}$, $C$: $\mathsf{int} \rightarrow \mathsf{bool}$) : $\mathsf{\vset{}}$\\ 
 Given a \vset{} $U$, returns a \vset{} $U'$ containing all $v$ such that $(u, v) \in E$ for $u \in U$ and $C(v) = \emph{true}$ and $F(u, v) = \emph{true}$.

 \smallskip



\subsection{Implementation}\label{sec:implementation}

We now describe how the framework can be implemented using
\treepluses{}. All of our implementations are written in C++, although
our ideas are more general and should easily translate to
a purely-functional language, like ML. Our
implementations use a custom pool-based memory allocator instead
of calling malloc and free. The pool-allocation is critical for
achieving good performance due to the large number of small memory
allocations that are made for tree nodes and \chunks{} in our
algorithms.

\myparagraph{\treeplus{} Implementation}
The underlying purely-functional tree data structure which we use in
our implementations is based on PAM~\cite{sun2018pam}. Our \treeplus{}
implementation is a little over 1000 lines of code, with most of the
code being due to the \textsc{Split}, \textsc{Union},
\textsc{Difference}, and \textsc{Intersection} implementations described in the supplementary material.

\myparagraph{Graph Implementation}
We implemented the graph data structure described in
Section~\ref{sec:graphsastrees} using a purely-functional tree to
represent the \vtree{}, and a \treeplus{} for each \etree{}. We note
that in principle it should be possible to implement the \vtree{}
using a \treeplus{}, which may improve compression and locality even
further. The graph data structure only required a few hundred lines of
code. We also implemented a simple version of the graph data structure
using nested purely-functional trees, which required a few dozen lines
of code.

\myparagraph{\textsc{Acquire} and \textsc{Release} Implementation}
Our approach for implementing these primitives is based on the
recently defined \emph{version maintenance
problem}~\cite{ben2018efficient}. This is the problem of maintaining a
multi-versioned object in a setting where a single writer updates the
object, creating new versions, while multiple readers can be reading
potentially different versions of the object. The authors
of~\cite{ben2018efficient} describe a simple, lock-free algorithm
which we implemented in a few dozen lines of code, although the details
are out of scope of this paper. The implementation guarantees strict
serializability, which in our setting means that the state of the
graph and outputs of queries are consistent with some serial execution
of the updates and queries corresponding to real time.


%% We start our implementation description by introducing
%% We now describe how the interface is implemented, and the theoretical
%% guarantees on work and depth provided by our implementation for each
%% of the primitives. We start
% \input{version-maintenance}


%% \myparagraph{Implementation}
%% %% We note that this graph data structure can be implemented cleanly in
%% %% about 100 lines of code using existing libraries for maintaining
%% %% purely functional trees under batch-insertions and batch-deletions,
%% %% such as PAM.
%% We implemented both the simple data structure and the \treeplus{} data
%% structure using PAM~\cite{sun2018pam}. The simple trees required about
%% 100 lines of code and served as a useful baseline. The \treeplus{}
%% implementation is a little over 1000 lines of code, with most of the
%% code being due to the \textsc{Split}, \textsc{Union},
%% \textsc{Difference}, and \textsc{Intersection} implementations.
%% %% \julian{which simple approach is this referring to?}
%% %% The interested reader can find proofs of the work-depth
%% %% bounds in~\cite{blelloch16justjoin} and details about augmented trees
%% %% in~\cite{sun2018pam}.
%%

%% \subsection{Versioned Graphs}
%% We describe algorithmic details about the data structures employed by
%% our framework in Section~\ref{sec:trees}. Here, we go over how the
%% main components of our framework can be easily implemented using the
%% version maintenance primitives described in
%% Section~\ref{sec:versions}. Assuming a primitive to generate the
%% initial $\version{}$ of a $\versionedgraph{}$, \buildgraph{} simply
%% returns the initial graph as the first version in the version
%% maintenance data structure.  \acquire{} and \release{} are easily
%% implemented using the \acquirev{} and \releasev{} primitives from
%% Section~\ref{sec:versions}. Finally, the primitives for mutating the
%% graph work by acquiring the latest graph, modifying it using the
%% primitives defined in Section~\ref{sec:trees} and making the new
%% version of the graph visible using \setv{}.
%% Queries are run on immutable versions of the graph, which guarantees strict serializability.


==> inputs/ideas.tex <==
\section{Rough ideas}

\subsection{Precise GC for version-controlled vertices}
Not linking the graph up as a persistent data-structure could be useful as it
lets readers of a vertex avoid an $O(\log n)$ lookup when finding the
vertex-root. The ``usual'' case (we could try to formalize this analytically)
touches a vertex that is infrequently updated, so there should be very few
versions on it, and finding the correct version should be easy.

One interesting question is how to provide precise GC even in this case when
vertex-roots with timestamp $T$ are not linked up by a tree associated with that
version. Recall that by \emph{precise}, we mean that no versions are held onto
that are not the active version, or are visible to an active transaction.

\myparagraph{Amortized collection}
Here's a simple idea: keep up to $2P$ versions per vertex. Once we hit $2P$
versions, we know that only $P$ of them can actually be live, so we will get rid
of at least $P$ of them. We do a read of the $P$ live transactions and their ids
at this moment and check for each versions whether it is still visible by a live
transaction, keeping it if it is, and discarding it if it isn't. One possible
implementation of this step running in $O(\log P)$ per version is to first sort
the versions by timestamp, then look-up for each versions whether it is visible,
marking it with the timestamp of the first reader it is visible to. We then just
remove contiguous runs with the same reader-timestamp, keeping only the latest
write that is visible to that reader.  As there are $\leq P$ active readers at
all times, it's easy to argue that we get rid of half of the versions, which
gives us our bound of $O(\log P)$ for garbage-collection per vertex-root.

Note that the garbage-collection here is not precise (we may hold onto versions
long after they become invisible). In fact, I'm not really sure what we can say
in terms of the total amount of space wasted by this approach. I think that it
is upper-bounded by the sum of the maximum amount of space over any length-$P$
window of versions for a particular vertex.

\myparagraph{Precise collection}
The only event that can trigger a version to need to be collected is when it is
\emph{currently} the current version that is now being replaced by a newer
version. In this case, we know that we will eventually say goodbye to this
version; it may be needed for now because of some active transactions that is is
(possibly) visible to, but will eventually become collectable once all of these
active transactions finish. The idea is to take advantage of this point in time
when a current verion is getting the boot to tag it in some structure so that
we can easily collect it once all of the timestamps it is visible to are done.

We will maintain a balanced BST on \emph{timestamps} that are currently active
(associated with an active reader). A node for a new timestamp is inserted as a
leaf when the timestamp is first made visible (\emph{before?} need to figure out).
Now, each active transaction (when it serializes and acquires a TS), does
nothing in the tree, as the timestamp is already considered active. When a
transaction finishes, calls \textsc{release}, and gets back \emph{true}, then
we know that this timestamp is dead. In this case, we delete the node from the
tree, check whether it was the only child of its parent, and if so delete the
parent as well (we don't delete the root).

The idea is to associate with each interval in the tree a set of vertex-roots
that can be collected once all timestamps in that interval are dead. The
responsibility of the writer when replacing versions is to stick a replaced
version in the set of the correct interval. The responsibility of a reader that
receives a \emph{true} from \textsc{release} is to delete (recursively) from
this tree, calling \textsc{collect} on all intervals that are newly dead on its
death.

Assuming that all of the above works, we should be able to prove that we can get
precise GC while paying $O(\log P)$ per vertex-root.

I'm not sure what datastructure this BST should be stored in. Probably a
concurrent skip-list?


==> inputs/implementations.tex <==
\section{Optimizations}\label{sec:optimizations}
%% In this section we briefly describe the algorithms and additional optimizations
%% we implemented in Aspen.

%% \myparagraph{Local and Global Algorithms, Flat Snapshots}
%% Notice that algorithms in our framework that use \emap{} incur an
%% extra $O(K \log n)$ factor in their work, where $K$ is the total
%% number of vertices accessed by \emap{} over the course of the
%% algorithm. For an algorithm like breadth-first search, which runs in
%% $O(m + n)$ work and $O(\mathsf{diam}(G) \log n)$ depth using a
%% static-graph processing framework~\cite{dhulipala2018theoretically}, a
%% naive implementation using our framework will require performing $O(m
%% + n\log n)$ work (the depth, however, is the same).
%%
%% Instead, for \emph{global graph algorithms}, which we loosely define
%% as performing at least $O(n)$ work, we can afford to take a \emph{flat
%% snapshot} of the graph, which reduces the $O(K \log n)$ term to
%% $O(K)$. The idea of a flat snapshot is very simple---instead of
%% accessing vertices through the vertex tree, and calling \textsc{Find}
%% for each $v$ supplied to \emap{}, we just precompute the edges tree
%% for all $v \in V$ and store handles to the trees in an array of size
%% $n$. By providing this array, which we call a \defn{flat snapshot} to
%% each call to \emap{}, we can directly access the edges tree in $O(1)$
%% work and reduce the work of \emap{} on a \vset{}, $U$, to $O(\sum_{u\in
%% U}\emph{deg}(u) + |U|)$.
%%
%% On the other hand, for \emph{local graph algorithms}, which perform
%% $o(n)$ work, we cannot afford to take a flat snapshot, as it will
%% affect the work of the algorithm asymptotically, possibly by much more
%% than an $O(\log n)$ factor. For these algorithms, we pay the cost of
%% traversing the vertex tree, but note that even these algorithms could
%% potentially be optimized by caching results from the vertex tree in
%% order to exploit temporal locality (this could likely be used to speed
%% up the Nibble algorithm). We discuss the benefit provided by flat
%% snapshots in the supplementary material.
%% % We experimentally verify the benefit
%% % provided by taking a flat snapshot in Section~\ref{sec:exps}.
%%
%% \myparagraph{Direction Optimization}
%% Aspen supports direction optimization,
%% an optimization technique first described for breadth-first search in
%% Beamer et al.~\cite{beamer12direction}, and later generalized as part
%% of Ligra~\cite{shun2012ligra}. We were able to easily
%% implement the optimization in Aspen by implementing a sparse version
%% and dense version of \emap{} by traversing the underlying
%% \treepluses{}. Aspen also supports an alternate dense implementation
%% called \textsc{DenseForward} that is implemented in Ligra, which scans
%% all edges incident to the current frontier and writes the output to a
%% dense vector.

\myparagraph{Implementation}
%% We note that this graph data structure can be implemented cleanly in
%% about 100 lines of code using existing libraries for maintaining
%% purely functional trees under batch-insertions and batch-deletions,
%% such as PAM.
We implemented both the simple data structure and the \treeplus{} data
structure using PAM~\cite{sun2018pam}. The simple trees required about
100 lines of code and served as a useful baseline. The \treeplus{}
implementation is a little over 1000 lines of code, with most of the
code being due to the \textsc{Split}, \textsc{Union},
\textsc{Difference}, and \textsc{Intersection} implementations.
%% \julian{which simple approach is this referring to?}
%% The interested reader can find proofs of the work-depth
%% bounds in~\cite{blelloch16justjoin} and details about augmented trees
%% in~\cite{sun2018pam}.


==> inputs/interface.tex <==
\section{An Interface for Dynamic Graphs}




==> inputs/new.tex <==
Due to the dynamic nature of real-world graphs, there has been a growing interest in the graph-streaming setting where a continuous stream of graph updates is mixed with arbitrary graph queries.  In principle, purely-functional trees are an ideal choice for this setting due as they enable safe parallelism, lightweight snapshots, and strict serializability for queries.  However, directly using them for graph processing would lead to significant space overhead and poor cache locality.


This paper presents C-trees, a compressed purely-functional search tree data structure that significantly improves on the space usage and locality of purely-functional trees. The key idea is to use a chunking technique over trees in order to store multiple entries per tree-node. We design theoretically-efficient and practical algorithms for performing batch updates to C-trees, and also show that we can store massive dynamic real-world graphs using only a few bytes per edge, thereby achieving space usage close to that of the best static graph processing frameworks.

To study the efficiency and applicability of our data structure, we designed Aspen, a graph-streaming framework that extends the interface of Ligra with operations for updating graphs.  We show that Aspen is faster than two state-of-the-art graph-streaming systems, Stinger and LLAMA, while requiring less memory, and is competitive in performance with the state-of-the-art static graph frameworks, Galois, GAP, and Ligra+.  With Aspen, we are able to efficiently process the largest publicly-available graph with over two hundred billion edges in the graph-streaming setting using a single commodity multicore server with 1TB of memory.



==> inputs/roadmap.tex <==
\section{Roadmap}




==> inputs/simple-trees.tex <==
%\subsection{Simple Tree-Based Data Structure}
\subsection{Graphs Using Trees}
\label{sec:simple-trees}

%\julian{I think we assumed in prelims that we are working with simple graphs. Not sure if it is worth differentiating simple and multigraphs in this paper}
%\laxman{Sounds good---I got rid of the discussion about multigraphs}

%\julian{``nodes'' is overloaded in this paper. we should refer to vertices in a graph as vertices and nodes in the tree as nodes.}
%\laxman{Makes sense!}

% This section introduces the main ideas. Show how to insert and
% delete edges from the tree using tree-union and tree-difference.

% \laxman{Figure showing how to represent a graph as a tree of
% vertices containing a tree of edges}
% \laxman{Figure showing how updating an edge just requires path copying
% and incrementing the ref-counts of nodes adjacent to the path}


\begin{figure*}[!t]
    \includegraphics[width=0.9\textwidth]{figures/simple-tree}\\ 
    \caption{\small We illustrate how the graph (shown on the left in
    green) is represented as a simple tree of trees (in the middle)
    and as a tree of \treepluses{} (on the right). In both
    representations we focus on the tree (\treeplus{}) for vertex 2.
    For the \treeplus{}, notice that only vertices 1 and 2 are
    selected as heads, so all of the remaining vertex IDs either
    appear in the tail of some node in the \treeplus{}, or in the
    \plus{}.}\label{fig:tree-of-trees}
  %\vspace{-1em}
\end{figure*}

An undirected graph can be implemented using purely
functional tree-based data structures by representing the set of
vertices as a tree, which we call the \defn{vertex tree}. Each vertex
in the vertex tree represents its adjacency information by storing a tree of
identifiers of its adjacent neighbors, which we call the \defn{edge
tree}. Directed graphs can be represented in the same way by
simply storing two edge trees per vertex, one maintaining the
out-neighbors, and one for the in-neighbors. The resulting graph data
structure is a tree-of-trees that has $O(\log n)$ overall depth using
a balanced tree implementation. Figure~\ref{fig:tree-of-trees}
illustrates the vertex tree and the edge trees for an example graph.
We augment the nodes of the trees with the number of
edges in the subtree.
In our implementation we use augmented maps and sets from PAM for the
trees---sets of vertex identifiers for the edge-tree, and a map from
vertex identifier to edge-tree for the vertex tree.

%\julian{A figure showing the tree of trees structure would be helpful. It can be placed next to a figure showing the tree of tree-pluses}

%% \myparagraph{Data Structure}
%% We now describe how we can use ordered maps (see
%% Section~\ref{sec:prelims}) to represent undirected, unweighted graphs.
%% %% \julian{drop ``simple''? also we don't have the PAM interface in prelims, so maybe reword}
%% We represent edge trees (the neighbors of a vertex) using an
%% \textsc{int} ordered set. We assume that each vertex is uniquely
%% identified by an integer id. We augment the set by setting the base
%% value for each key to $1$, and combining values using $+$ with $0$ as
%% the identity, which lets us maintain the degree of the vertex by
%% computing the augmented value of the map.

%% A Graph is represented as a vertex tree, which is an ordered map over
%% vertices where the keys are \textsc{Int} vertex identifiers and the
%% values are edge trees. To efficiently maintain the number of edges in
%% the graph while the graph changes, we augment the map by taking the
%% base value for each key as the degree of the vertex, and combining
%% values using $+$ and $0$ as the combine function and identity,
%% respectively. Weights can be represented by changing the edge
%% tree from an ordered set to an ordered map and storing the weights as
%% values.

%% \julian{why is the original set unordered but the map ordered?}
%% \laxman{changed `set' to `ordered set' (not sure if it's redundant,
%% but it's more clear, at least to me). We can move the sentence about
%% what an ordered set is to the prelims.}

% \myparagraph{Implementing the Aspen Interface}

We implement \textsc{NumVertices} and \textsc{NumEdges} by returning the size (number of keys) in the vertex tree and the
augmented value of the vertex tree respectively, which can be done in
$O(1)$ work. \textsc{FindVertex} takes a vertex ID and
searches the vertex tree, which takes $O(\log n)$ work and depth.
We implement \textsc{EdgeMap} by mapping over the vertices in the
input \vset{} $U$ in parallel and for each vertex $u \in U$ searching the vertex
tree for its edge-tree, and then mapping over $u$'s incident
neighbors, again in parallel.  For each of $u$'s neighbors $v$ we
apply the map function $F(u,v)$ if the filter function $C(u,v)$
returns true.  Other than finding vertices in the input \vset{} in $G$
and traversing edges via the tree instead of an array, the
implementation is effectively the same as in
Ligra~\cite{shun2012ligra}.  We note that the direction
optimization~\cite{beamer12direction,shun2012ligra} can be implemented
using this data structure, and we describe more details in
Section~\ref{sec:optimizations}.  Assuming the functions $F$ and $C$
take constant work, \textsc{EdgeMap} takes
$O(\sum_{u\in U}\emph{deg}(u) + |U|\log n)$ work and $O(\log n)$ depth.

\textsc{InsertEdges} and \textsc{DeleteEdges} are similar, and so we only
provide details for \textsc{InsertEdges}. Let $A$ be the sequence
(batch) of edge updates and let $k = |A|$.  We first sort the batch of
edge pairs using a comparison sort.  We then compute an array of
source vertex IDs that are being updated and for each, in parallel, we
build a tree over its target vertices using \textsc{Build}.  This
creates a sequence of vertex-tree pairs representing each source
vertex to be updated along with a tree of its target vertices to be
updated.  The last step is to call \textsc{MultiInsert} to insert the
new entries.  The combine function for \textsc{MultiInsert} combines
existing values (trees of edges) with the new trees by calling
\textsc{Union}.

All operations before the \textsc{MultiInsert} can be done in $O(k \log k)$
work and $O(\log k)$ depth.
The work and depth of the \textsc{MultiInsert} can be easily
upper-bounded as $O(k \log n)$ and $O(\log^3 n)$, but the actual
bounds can be be much better.  Let $v_i$ be the $i$'th vertex in $L$
and $s_i = \min(d_{L}(v_i), d_{G}(v_i))$ and $t_i = \max(d_{L}(v_i),
d_{G}(v_i))$. We define $s_i = t_i = 1$ if $v_i$ is not present in
$G$. Let $q = \min(|L|, n), r = \max(|L|, n)$.  The work of the
\textsc{MultiInsert} is
\begin{equation*}
  O\left(q \log \left(\frac{r}{q} + 1\right) + \sum_{i=0}^{|L|} s_i \log
  \left(\frac{t_i}{s_i} + 1\right)\right)
\end{equation*}
where the first term is from the bound on \textsc{MultiInsert}, and
the second term accounts for the cost of performing \textsc{Union} on
each updated vertex.  Notice that when each existing vertex receives a
number of updates proportional to its current degree, the overall work
over the \textsc{MultiInsert} is $O(q \log (\frac{r}{q} + 1))$, which
becomes $O(n)$ once a constant fraction of the vertices are
updated. In the worst case, the first term is $O(k \log n)$ and the
second term is also $O(k \log n)$. The depth of the
\textsc{MultiInsert} is  $O(\log n  (\log m + D_{\textsc{Union}}(v_{L}, v_{G})))$
which simplifies to $O(\log^3 n)$ by upper-bounding
$D_{\textsc{Union}}(v_{L}, v_{G})$ as $O(\log^2 n)$.

%% The vertex primitives in Table~\ref{table:graphinterface} are easily
%% implemented using the corresponding operations on trees (see
%% Figure~\ref{fig:mapinterface}).

%% \julian{do we support inserting vertices? if so, add description}
%% \laxman{todo: add vertex description, fix notation bugs above}



==> inputs/version-maintenance.tex <==
%\subsection{Version Maintenance}\label{sec:versions}
\myparagraph{Version Maintenance}
The \defn{version maintenance problem}~\cite{ben2018efficient} is the
problem of maintaining a multi-versioned object in a setting where a
single writer updates the object, creating new versions, while multiple
readers can be reading potentially different versions of the object.
The problem was introduced and studied very recently by Ben-David et
al.~\cite{ben2018efficient} to obtain practical algorithms for
multi-versioned objects in the single-writer setting.

Formally, the problem is to provide transactional guarantees for the
following operations: \defn{\acquirev{}}, \defn{\releasev{}}, and
\defn{\setv{}}. \acquirev{} and \releasev{} are used by readers to
acquire a new version of the data structure in a read-only state and
to release it once it is finished being used. \setv{} is used by the
single writer in order to make a new version of the object available
to readers. In Aspen, we implemented the lock-free algorithm described
in~\cite{ben2018efficient}, which guarantees strict serializability
for the operations above, and precise garbage collection (roughly,
versions which are no longer being read are immediately collected).
In our setting, strict serializability means that the state of the
graph and outputs of queries are consistent with some serial execution of the updates and queries corresponding to real time.
We provide implementation details in the full version of the paper, as
this algorithm is not a contribution of this paper.


%% In this paper we implemented the lock-free algorithm presented
%% in~\cite{ben2018efficient}, which guarantees strict serializability
%% for the operations listed above, and precise garbage collection
%% (roughly, version which are no longer being read are immediately collected).
%% The main data structure in the implementation is a hash table of size
%% $O(P)$, where $P$ is the number of processors. The keys are
%% timestamps, and the values are pairs of versions and reference-counts.
%% We assume that each processor views at most one version, but this
%% assumption can be easily relaxed to enable processing multiple views
%% of the graph in time. To implement \acquirev{} the reader reads the
%% global timestamp, searches the hash-table for the version, and then
%% atomically increments the reference count using a fetch-and-add
%% operation. If the value returned is 0, then it has already been
%% released by all reading processors (and is no longer the latest
%% version), so the processor tries again.  Otherwise, the version is
%% valid, and so we return it.  To implement \setv{}, the writer first
%% reads the current version using \acquirev{}, makes modifications to
%% generate a new version, and then inserts the new version into the
%% table with a reference-count of 1. It then atomically increments the
%% global timestamp, making hte new version visible. Finally, the writer
%% calls \releasev{} on the previous version.

